When Policies Cannot Be Retrained: A Unified Closed-Form View of Post-Training Steering in Offline Reinforcement Learning

Offline reinforcement learning (RL) can learn effective policies from fixed datasets, but deployment objectives may change after training, and in many applications the trained actor cannot be retrained because of data, cost, or governance constraints. We study deployment-time adaptation for frozen offline actors using Product-of-Experts (PoE) composition with a goal-conditioned prior. Our main practical finding is graceful degradation rather than universal performance gain: under degraded or random priors, precision-weighted composition remains anchored to the frozen actor, while additive and prior-only adaptation collapse, and a KL-budget selector often recovers a near-oracle operating point. We also make explicit a closed-form identity in the frozen-actor setting: for diagonal-Gaussian actors and priors, PoE with coefficient alpha yields the same deterministic policy as KL-regularized adaptation with beta = alpha / (1 - alpha), with posterior covariances differing only by a global scalar factor. Empirically, across four D4RL environments (3,900 MuJoCo episodes), we observe a 4/5/3 HELP/FROZEN/HURT split. Extending the analysis to six harder cells and two AntMaze diagnostics reveals an actor-competence ceiling: medium-expert remains HURT in all 9 cells at every tested alpha, while AntMaze with a behavior-cloned frozen actor yields zero success for all composition rules. Overall, PoE and KL-regularized adaptation are best viewed as a single actor-anchored safety mechanism for deployment-time steering.

==> checklist.tex <==
\section*{NeurIPS Paper Checklist}

\begin{enumerate}

\item {\bf Claims}
    \item[] Question: Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \item[] Answer: \answerYes{}
    \item[] Justification: The abstract and introduction state the core contributions, each directly supported by the evidence package. The closed-form equivalence $\mathrm{PoE}(\alpha)\equiv\mathrm{KL\text{-}Reg}(\beta=\alpha/(1-\alpha))$ is derived in Sec.~\ref{sec:equivalence} and verified on dataset states and MuJoCo rollouts in Sec.~\ref{sec:d4rl_equivalence} / Appendix~\ref{app:equivalence_audit}. The empirical characterization claim (help on $4$ of $12$ cells, frozen on $5$, hurt on $3$; robustness under degraded priors) is substantiated in Sec.~\ref{sec:d4rl_headline} and Sec.~\ref{sec:d4rl_prior_robustness_main}, with per-cell numbers in \texttt{outputs/rollout/\_paper/main\_results\_table.csv}, \texttt{diagnostic\_summary.csv}, and \texttt{prior\_degradation\_table.csv}. The harder-regime claim (medium-expert uniformly \textsc{Hurt} at every $\alpha$ we tested, medium-replay recovering Frozen ties as $\alpha$ rises) is substantiated by the $\alpha$ sweep in Sec.~\ref{sec:harder_regimes} and Appendix~\ref{app:harder_alpha_sweep}, with per-cell numbers in \texttt{outputs/d4rl/harder\_alpha\_sweep/best\_alpha\_per\_cell.csv} and verdict counts in \texttt{outputs/d4rl/harder\_alpha\_sweep/verdict\_by\_regime\_alpha.csv}. The AntMaze boundary claim (zero success with a BC frozen actor across all methods) is supported by Appendix~\ref{app:antmaze_diagnostic} and the rollout CSVs under \texttt{outputs/d4rl/antmaze\_rollout\_full/antmaze-umaze-v2/} and \texttt{outputs/d4rl/harder\_regime\_rollout\_full/antmaze-medium-play-v2/}. We state explicitly that composition does not universally improve over the frozen actor (including the stronger ceiling on medium-expert) and that Theorem~\ref{thm:cpi} is qualitative at $\gamma=0.99$, not predictive.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the abstract and introduction do not include the claims made in the paper.
        \item The abstract and/or introduction should clearly state the claims made, including the contributions made in the paper and important assumptions and limitations.
        \item The claims made should match theoretical and experimental results.
        \item It is fine to include aspirational goals as motivation as long as it is clear that these goals are not attained by the paper.
    \end{itemize}

\item {\bf Limitations}
    \item[] Question: Does the paper discuss the limitations of the work performed by the authors?
    \item[] Answer: \answerYes{}
    \item[] Justification: An explicit Limitations paragraph closes Sec.~\ref{sec:conclusion}: (i)~composition can hurt on speed-dominant goals where the frozen actor is already near its behavioral ceiling ($3$ of $12$ main-body cells); (ii)~Theorem~\ref{thm:cpi}'s penalty coefficient $2\gamma/(1-\gamma)^2=19{,}800$ at $\gamma=0.99$ and the sup-state total-variation that saturates near $1$ make the right-hand side of Eq.~\eqref{eq:cpi-bound} loose, so we treat it as a structural decomposition only; (iii)~the AWR/AWAC critic-gradient baseline is trained by fitted-Q evaluation without conservative regularization, while CQL/IQL-guided critics are appendix-only comparison baselines and remain mixed; an SF/GPI baseline is also appendix-only (Appendix~\ref{app:sf_gpi}) and does not displace density-anchored composition; (iv)~the evaluation budget is $5$ seeds $\times\,5$ episodes per cell on the main package and the harder-regime package. We additionally state an \emph{actor-competence ceiling}: on medium-expert every $\alpha\in\{0.1,0.3,0.5,0.7,0.9\}$ yields \textsc{Hurt} in every cell we tested, and on \texttt{antmaze-umaze-v2}/\texttt{antmaze-medium-play-v2} with a BC frozen actor every method returns zero (Appendix~\ref{app:antmaze_diagnostic}); we do not probe $\alpha>0.9$ and we do not claim the frozen-actor paradigm applies to AntMaze-grade exploration. The \textsc{Help}/\textsc{Frozen}/\textsc{Hurt} classifier is documented in Appendix~\ref{app:diagnostic}.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the paper has no limitation while the answer \answerNo{} means that the paper has limitations, but those are not discussed in the paper.
        \item The authors are encouraged to create a separate ``Limitations'' section in their paper.
        \item The paper should point out any strong assumptions and how robust the results are to violations of these assumptions.
        \item The authors should reflect on the scope of the claims made, e.g., if the approach was only tested on a few datasets or with a few runs.
    \end{itemize}

\item {\bf Theory assumptions and proofs}
    \item[] Question: For each theoretical result, does the paper provide the full set of assumptions and a complete (and correct) proof?
    \item[] Answer: \answerYes{}
    \item[] Justification: Theorem~\ref{thm:variational} (KL-barycenter identity) is stated with its finite-action and bounded-log-density assumptions and proved in Appendix~\ref{app:proof-theorem1}. Theorem~\ref{thm:cpi} (performance-difference decomposition) relies on two standard lemmas (performance-difference and discounted occupancy perturbation) collected in Appendix~\ref{app:auxiliary-lemmas} and proved in Appendix~\ref{app:proof-theorem-2}. Theorem~\ref{thm:robustness} (transition shift) is proved in Appendix~\ref{app:proof-theorem-3}, with its supporting kernel-shift lemma in Appendix~\ref{app:auxiliary-transition-shift}. Proposition~\ref{prop:interp} (interpolation and support preservation) and its proof are in Appendix~\ref{app:proof-proposition1}. The continuous-action Wasserstein statement of Proposition~\ref{prop:gaussian-poe-bound} and Corollary~\ref{cor:gaussian-poe-kl} is proved in Appendix~\ref{app:theory-continuous}. Corollaries~\ref{cor:improve}, \ref{cor:deploy}, and \ref{cor:plugin} are in Appendices~\ref{app:proof-corollary-1}, \ref{app:proof-corollary-2}, and \ref{app:proof-corollary-3}. We explicitly state that Theorem~\ref{thm:cpi} is not a predictive bound at $\gamma=0.99$ (Appendix~\ref{app:cpi_diagnostic}).
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the paper does not include theoretical results.
        \item All the theorems, formulas, and proofs in the paper should be numbered and cross-referenced.
        \item All assumptions should be clearly stated or referenced in the statement of any theorems.
        \item Theorems and Lemmas that the proof relies upon should be properly referenced.
    \end{itemize}

    \item {\bf Experimental result reproducibility}
    \item[] Question: Does the paper fully disclose all the information needed to reproduce the main experimental results of the paper?
    \item[] Answer: \answerYes{}
    \item[] Justification: Appendix~\ref{app:reproducibility} documents the frozen rollout evidence package. It records the git commit hash, hostname, Python and package versions (PyTorch, NumPy, pandas, SciPy, gym, mujoco, \texttt{mujoco\_py}, D4RL), GPU driver and model, and the SHA-256 digest of every evidence CSV. The pipeline is wrapped in \texttt{scripts/run\_main\_rollouts.sh} ($5$ seeds $\times$ $5$ episodes $\times$ $3$ goals $\times$ $4$ environments, $3{,}900$ episodes), \texttt{scripts/run\_prior\_degradation.sh} ($3$ seeds $\times$ $3$ episodes $\times$ $3$ goals $\times$ $4$ environments $\times$ $4$ prior variants, $2{,}160$ episodes), and \texttt{scripts/run\_adaptive\_alpha\_suite.sh} for the practical alpha-selection study. The appendix-only CQL/IQL sweep is released under \texttt{outputs/d4rl/cql\_iql\_rollout\_paper2/} together with a paper table builder at \texttt{experiments/d4rl/build\_cql\_iql\_tables.py}. The harder-regime and $\alpha$-sweep packages are produced by \texttt{scripts/train\_and\_rollout\_env.sh}, \texttt{scripts/chain\_envs.sh}, and \texttt{scripts/alpha\_sweep\_env.sh}; outputs live under \texttt{outputs/d4rl/harder\_regime\_rollout\_full/}, \texttt{outputs/d4rl/harder\_alpha\_sweep/}, and \texttt{outputs/d4rl/full\_harder\_benchmark/} with aggregation via \texttt{scripts/aggregate\_rollouts.py} and analysis via \texttt{scripts/analyze\_alpha\_sweep.py}; a per-env runbook is at \texttt{scripts/RUNBOOK\_harder\_benchmark.md}. A validator at \texttt{experiments/d4rl/validate\_rollout\_package.py} checks cell coverage, NaN counts, seed consistency, and the matched-pair equivalence on the main package and returns \texttt{STATUS: PASS}.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the paper does not include experiments.
        \item Reproducibility can be accomplished in various ways. Releasing code and data is one good way to accomplish this, but reproducibility can also be provided via detailed instructions for how to replicate the results.
    \end{itemize}


\item {\bf Open access to data and code}
    \item[] Question: Does the paper provide open access to the data and code, with sufficient instructions to faithfully reproduce the main experimental results?
    \item[] Answer: \answerYes{}
    \item[] Justification: We release the full code used to produce every evidence package, the raw rollout CSVs, per-seed summaries, aggregate tables, and all figures. Reproducibility instructions for the four-env main-body package are in Appendix~\ref{app:reproducibility} and the top-level scripts \texttt{scripts/run\_main\_rollouts.sh}, \texttt{scripts/run\_prior\_degradation.sh}, and \texttt{scripts/run\_adaptive\_alpha\_suite.sh}. The appendix-only CQL/IQL sweep is released under \texttt{outputs/d4rl/cql\_iql\_rollout\_paper2/}. The harder-regime + $\alpha$-sweep package is produced by \texttt{scripts/train\_and\_rollout\_env.sh}, \texttt{scripts/chain\_envs.sh}, and \texttt{scripts/alpha\_sweep\_env.sh}, with outputs under \texttt{outputs/d4rl/harder\_regime\_rollout\_full/} and \texttt{outputs/d4rl/harder\_alpha\_sweep/}; aggregation via \texttt{scripts/aggregate\_rollouts.py} and interpretation via \texttt{scripts/analyze\_alpha\_sweep.py}. The AntMaze diagnostic package is under \texttt{outputs/d4rl/antmaze\_rollout\_full/}. The D4RL datasets (\texttt{halfcheetah/hopper/walker2d-medium-v2}, \texttt{-medium-replay-v2}, \texttt{-medium-expert-v2}, \texttt{antmaze-umaze-v2}, \texttt{antmaze-medium-play-v2}) are accessed through the standard D4RL release; dataset manifest at \texttt{configs/d4rl\_dataset\_manifest.json}.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that paper does not include experiments requiring code.
        \item The instructions should contain the exact command and environment needed to run to reproduce the results.
    \end{itemize}


\item {\bf Experimental setting/details}
    \item[] Question: Does the paper specify all the training and test details necessary to understand the results?
    \item[] Answer: \answerYes{}
    \item[] Justification: Sec.~\ref{sec:setup} specifies the main-body environments, the actor and prior architectures (diagonal-Gaussian, behavioral cloning for the actor, contrastive goal-weighted BC for the prior), the deployment-goal definitions $G_1=(1,0.1,0.1)$, $G_2=(0.5,0.5,0.5)$, $G_3=(0.1,1,0.1)$, the evaluation protocol (real MuJoCo rollouts, $5$ seeds, $5$ episodes per seed), the reward-component decomposer shared between prior training and rollout evaluation, and the method set with matched $\alpha$ and $\beta=\alpha/(1-\alpha)$. The KL-Reg $\beta$ grid is $\{0.111,0.429,1.000,2.333,9.000\}$ and the PoE $\alpha$ grid is $\{0.1,0.3,0.5,0.7,0.9\}$. Sec.~\ref{sec:harder_regimes} and Appendix~\ref{app:harder_rollouts} specify the additional harder-regime envs (\texttt{halfcheetah/hopper/walker2d-medium-replay-v2} and \texttt{-medium-expert-v2}) and AntMaze diagnostic envs (\texttt{antmaze-umaze-v2}, \texttt{antmaze-medium-play-v2}); they reuse the same actor / prior / critic training recipes, with AntMaze using the \texttt{\{G1\_success, G2\_balanced, G3\_efficient\}} goal scheme described in the AntMaze reward decomposer. Full per-cell hyperparameters and training scripts are in Appendix~\ref{app:training-setup}.
    \item[] Guidelines:
    \begin{itemize}
        \item The experimental setting should be presented in the core of the paper to a level of detail that is necessary to appreciate the results.
    \end{itemize}

\item {\bf Experiment statistical significance}
    \item[] Question: Does the paper report error bars suitably and correctly defined or other appropriate information about the statistical significance of the experiments?
    \item[] Answer: \answerYes{}
    \item[] Justification: Headline results in Sec.~\ref{sec:d4rl_headline} and Figure~\ref{fig:headline_rollout} carry $95\%$ bootstrap confidence intervals computed over $25$ episodes per (method, environment, goal) cell, resampled from per-seed summaries. The \textsc{Help}/\textsc{Frozen}/\textsc{Hurt} classifier in Appendix~\ref{app:diagnostic} uses one confidence-interval half-width as its threshold. The equivalence claim in Sec.~\ref{sec:d4rl_equivalence} is supported by seed-matched paired comparisons at each matched $\alpha$ with $95\%$ bootstrap CIs on the paired difference, and by rliable-style probability of improvement~\citep{agarwal2021deep}. All intervals are empirical resampled intervals; we do not assume Gaussian error distributions.
    \item[] Guidelines:
    \begin{itemize}
        \item The authors should answer \answerYes{} if the results are accompanied by error bars, confidence intervals, or statistical significance tests.
        \item The method for calculating the error bars should be explained.
    \end{itemize}

\item {\bf Experiments compute resources}
    \item[] Question: Does the paper provide sufficient information on the computer resources needed to reproduce the experiments?
    \item[] Answer: \answerYes{}
    \item[] Justification: Appendix~\ref{app:reproducibility} records the observed wall times on the hardware we used. The full main rollout pipeline (four environments, five seeds, five episodes, three goals, thirteen methods) completed in approximately $35$ minutes on a single NVIDIA TITAN RTX. The prior-degradation pipeline (four environments, three seeds, three episodes, three goals, five methods, four prior variants) completed in approximately $68$ minutes on the same hardware. The harder-regime + $\alpha$-sweep package completed in approximately $2.5$~hours on two NVIDIA TITAN RTX GPUs run in parallel, covering six locomotion envs and two AntMaze envs; the $\alpha$ sweep alone is $5{,}850$ episodes over six envs. GPU memory use peaked under $4$~GB per worker. All training (behavioral cloning for the actor, contrastive goal-weighted BC for the prior, FQE / CQL / IQL / SF critics) uses the same single-GPU setup.
    \item[] Guidelines:
    \begin{itemize}
        \item The paper should indicate the type of compute workers and memory used.
        \item The paper should provide the amount of compute required for each experiment.
    \end{itemize}

\item {\bf Code of ethics}
    \item[] Question: Does the research conducted in the paper conform with the NeurIPS Code of Ethics?
    \item[] Answer: \answerYes{}
    \item[] Justification: The work is performed entirely in the MuJoCo simulator on released D4RL datasets; it involves no human subjects, no scraped or sensitive data, and no deployment to real-world systems. The paper explicitly cautions in its discussion that post-training steering is not a substitute for re-validation when the updated objective is safety-relevant.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the authors have not reviewed the NeurIPS Code of Ethics.
    \end{itemize}


\item {\bf Broader impacts}
    \item[] Question: Does the paper discuss both potential positive societal impacts and negative societal impacts of the work performed?
    \item[] Answer: \answerYes{}
    \item[] Justification: The paper's motivation explicitly targets high-stakes deployment settings where retraining is blocked by governance, certification, revalidation, or cost constraints. The positive impact is a lightweight, interpretable actor-anchored composition layer that makes post-training steering auditable. The paper also discusses the negative failure mode: when the deployment prior is unreliable, naive composition (prior-only or additive) can silently degrade performance, and even precision-weighted composition can hurt on speed-dominant goals where the frozen actor is already near its behavioral ceiling. We emphasise that the method is a deployment-time steering mechanism and not a substitute for revalidating a policy whose deployment objective has changed in a safety-relevant way.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that there is no societal impact of the work performed.
    \end{itemize}

\item {\bf Safeguards}
    \item[] Question: Does the paper describe safeguards that have been put in place for responsible release of data or models that have a high risk for misuse?
    \item[] Answer: \answerNA{}
    \item[] Justification: The paper releases code and simulator-rollout result files for D4RL locomotion tasks. The artifacts pose no dual-use risk and carry no personal data. Model checkpoints are standard behavioral-cloning and Gaussian prior networks for public locomotion environments.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the paper poses no such risks.
    \end{itemize}

\item {\bf Licenses for existing assets}
    \item[] Question: Are the creators or original owners of assets used in the paper properly credited and are the license and terms of use explicitly mentioned and properly respected?
    \item[] Answer: \answerYes{}
    \item[] Justification: D4RL datasets~\citep{fu2020d4rl} and their environments are accessed through the official D4RL release under its stated license (Apache-2.0 for code, MIT for data). Underlying MuJoCo physics and \texttt{mujoco\_py} follow their respective licenses. PyTorch, \texttt{gym}, NumPy, SciPy, pandas, matplotlib, and seaborn are used under their respective open-source licenses. All cited methods are attributed in Sec.~\ref{sec:related-work}.
    \item[] Guidelines:
    \begin{itemize}
        \item The authors should cite the original paper that produced the code package or dataset.
        \item The name of the license should be included for each asset.
    \end{itemize}

\item {\bf New assets}
    \item[] Question: Are new assets introduced in the paper well documented and is the documentation provided alongside the assets?
    \item[] Answer: \answerYes{}
    \item[] Justification: We release the code for actor training, prior training, PoE and KL-regularized adaptation baselines, the matched-pair method-set builder, the rollout evaluator, the equivalence audit, and the CPI-bound diagnostic. We also release the frozen rollout evidence package (raw per-episode CSVs, per-seed summaries, aggregate summaries, paper-ready tables, equivalence audit, CPI diagnostic, reproducibility manifest with SHA-256 digests) under \texttt{outputs/rollout/}. Appendix~\ref{app:reproducibility} describes the layout and the scripts that produce each artifact.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the paper does not release new assets.
    \end{itemize}

\item {\bf Crowdsourcing and research with human subjects}
    \item[] Question: For crowdsourcing experiments and research with human subjects, does the paper include the full text of instructions given to participants and screenshots, if applicable, as well as details about compensation?
    \item[] Answer: \answerNA{}
    \item[] Justification: The paper does not involve crowdsourcing or research with human subjects. All experiments are performed in the MuJoCo simulator.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the paper does not involve crowdsourcing nor research with human subjects.
    \end{itemize}

\item {\bf Institutional review board (IRB) approvals or equivalent for research with human subjects}
    \item[] Question: Does the paper describe potential risks incurred by study participants, whether such risks were disclosed to the subjects, and whether Institutional Review Board (IRB) approvals were obtained?
    \item[] Answer: \answerNA{}
    \item[] Justification: The paper does not involve research with human subjects.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the paper does not involve crowdsourcing nor research with human subjects.
    \end{itemize}

\item {\bf Declaration of LLM usage}
    \item[] Question: Does the paper describe the usage of LLMs if it is an important, original, or non-standard component of the core methods in this research?
    \item[] Answer: \answerNA{}
    \item[] Justification: LLMs are not part of the core methodology. As noted in the existing AI usage statement in Appendix~\ref{app:ai-statement}, generative AI tools were used in a limited and supportive capacity during manuscript preparation and for code refactoring and formatting; all scientific content, experimental design, results, interpretations, and conclusions were conceived, implemented, and verified by the authors.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the core method development in this research does not involve LLMs as any important, original, or non-standard components.
    \end{itemize}

\end{enumerate}

